BindEnergyCraft: Casting Protein Structure Predictors as Energy-Based Models for Binder Design

Protein binder design has been transformed by hallucination-based methods that optimize structure prediction confidence metrics, such as the interface predicted TM-score (ipTM), via backpropagation. However, these metrics do not reflect the statistical likelihood of a binder-target complex under the learned distribution and yield sparse gradients for optimization. In this work, we propose a method to extract such likelihoods from structure predictors by reinterpreting their confidence outputs as an energy-based model (EBM). By leveraging the Joint Energy-based Modeling (JEM) framework, we introduce pTMEnergy, a statistical energy function derived from predicted inter-residue error distributions. We incorporate pTMEnergy into BindEnergyCraft (BECraft), a design pipeline that maintains the same optimization framework as BindCraft but replaces ipTM with our energy-based objective. BECraft outperforms BindCraft, RFDiffusion, and ESM3 across multiple challenging targets, achieving higher in silico binder success rates while reducing structural clashes. Furthermore, pTMEnergy establishes a new state-of-the-art in structure-based virtual screening tasks for miniprotein and RNA aptamer binders.

==> intro_AP.tex <==
\section{Introduction}

De novo protein binder design is a fundamental problem in molecular engineering and is key to developing targeted therapeutics, requiring sequences that both fold into stable structures and form high-affinity complexes with their targets. Recent advancements in deep-learning methods have enabled considerable progress in in-silico binder design, yet identifying high-affinity candidates still demands the generation and experimental screening of thousands of designs, posing a significant bottleneck for most research groups.

Current state-of-the-art methods like BindCraft use AlphaFold2-based hallucination to optimize the interface predicted TM-score (ipTM) as a proxy for binding affinity. However, ipTM is fundamentally limited as an optimization objective: its hard maximum operation produces sparse gradients, and it discards the rich distributional information in AlphaFold's confidence outputs. Alternative metrics either lack differentiability (Rosetta energy) or require computationally expensive dedicated models.

In our method, we observe that protein structure predictors implicitly define statistical energy functions through their confidence outputs. By applying the Joint Energy-based Model (JEM) framework—which shows that any classifier's logits can be interpreted as unnormalized energies—we extract a differentiable energy function from AlphaFold's predicted alignment error (pAE) distributions. Our pTMEnergy function aggregates inter-chain pAE logits using a physically-motivated LogSumExp operation, preserving gradient signal from all residue pairs rather than just the maximum. This formulation provides several key advantages: dense gradients that guide optimization across the full interface, continuous scores that avoid saturation, and a principled probabilistic interpretation as the likelihood of the complex under AlphaFold's learned distribution. Crucially, since pTMEnergy derives from the same pAE outputs as ipTM, it requires no additional forward passes or model modifications.

Integrating pTMEnergy into BindCraft's pipeline yields BindEnergyCraft (BECraft), which achieves higher in-silico success rates than BindCraft, RFDiffusion, and ESM-3 across diverse targets. Our analysis reveals that pTMEnergy engages 98-100\% of interface residues during optimization compared to 22-35\% for ipTM, explaining its improved performance and reduced susceptibility to adversarial local minima. Beyond design, pTMEnergy establishes state-of-the-art results in structure-based screening for both miniprotein binders and RNA aptamers. Moreover, having demonstrated the effectiveness of pTMEnergy as a versatile optimization objective, we anticipate broader utility in related contexts such as 

<any other contexts? want to express that this pTMEnergy ordeal is a concept, not just something we leverage here, meaning it can be applied to other contexts...  but also don't want to make any crazy claims>.

